Visual Distortions in 360-degree Videos

Omnidirectional (or 360-degree) images and videos are emergent signals in many areas such as robotics and virtual/augmented reality. In particular, for virtual reality, they allow an immersive experience in which the user is provided with a 360-degree field of view and can navigate throughout a scene, e.g., through the use of Head Mounted Displays. Since it represents the full 360-degree field of view from one point of the scene, omnidirectional content is naturally represented as spherical visual signals. Current approaches for capturing, processing, delivering, and displaying 360-degree content, however, present many open technical challenges and introduce several types of distortions in these visual signals. Some of the distortions are specific to the nature of 360-degree images, and often different from those encountered in the classical image communication framework. This paper provides a first comprehensive review of the most common visual distortions that alter 360-degree signals undergoing state of the art processing in common applications. While their impact on viewers' visual perception and on the immersive experience at large is still unknown ---thus, it stays an open research topic--- this review serves the purpose of identifying the main causes of visual distortions in the end-to-end 360-degree content distribution pipeline. It is essential as a basis for benchmarking different processing techniques, allowing the effective design of new algorithms and applications. It is also necessary to the deployment of proper psychovisual studies to characterise the human perception of these new images in interactive and immersive applications.

==> sections/1.intro.old.tex <==
\section{Introduction}
\label{sec:introduction}

360-degree Virtual Reality~(VR) videos are immersive spherical videos, mapped
onto a 3D geometry where the user can look around during playback using a VR
head-mounted display~(HMD). %~(see Fig.~\ref{fig:360video_overview}).
%%
It is currently a promising technology being pushed forward by major
standardization~\cite{hanhart2018360-degree} and industrial players, such as
Youtube and Facebook.
%%
To be successful, however, the overall infrastructure for 360 video ---which
includes capturing, representation, coding, transmission, rendering, and
visualization--- must support a good-enough quality of experience~(QoE) for
end users.

%\begin{figure}[!htb]
% \centering
% \includegraphics[width=0.2\textwidth]{imgs/hosseini2016_360video_overview.png}
% \caption{Visual structure of a 360 VR video.~\cite{hosseini2016adaptive}
%  \ranote{Remove this figure.}}
% \label{fig:360video_overview}
%\end{figure}

Compared to 2D conventional videos, 360-degree video pushes the current
storage and network capacities to their limits, especially since the 4K video
resolution is being widely accepted as a minimum functional resolution for
current HMDs, and 8K or higher is desired~\cite{hosseini2017view-aware}.
%%
Thus, new coding and networking techniques are needed to support a good-enough
QoE for 360 video end users.
%%
While watching a 360-degree video on a VR HMD, for instance, only a small
portion of the whole 360-degree screen is visible to the user at any given
point in time, which opens up many possibilities for improving the current
state-of-the-art approach of transmitting all the 360-degree video stream.

For evaluating those techniques and quantifying the visual quality of
360-degree immersive experiences, a deep understanding of the 360 processing
pipeline and the perceptible artifacts introduced by current approaches is
essential~\cite{desimone2017omnidirectional}.
%%
Indeed, the identification and classification of artifacts produced by state
of the art pipelines are essential to evaluate the performance of various
video coding software and hardware (products which are recently proliferating)
and for the effective design of high quality services.
%%
A comprehensive analysis and classification of the artifacts and its sources
has also the potential to assist in the design of more effective adaptive
quantization algorithms, coding mechanisms and post-processing techniques,
e.g., for minimizing or compensating the artifacts.

This paper focuses on the study of the perceptual artifacts on the 360 image
and video processing pipelines.
%%
Its main contribution is the identification and classification of visual
distortions occurring in an end-to-end 360-degree pipeline from capture,
coding, distribution, and visualization by the end user.
%Its main contribution is a comprehensive review of the artifacts that can
%occur on end-to-end pipelines for compressed 360-degree images and videos.
%%
The goal is the isolation of individual artifacts with the aim of obtaining a
description of the artifacts' visual manifestations, causes, and
relationships.
%%
Visual examples of the artifacts are presented when possible.

Although there have been similar works that categorize artifacts for planar 2D
conventional~\cite{yuen1998survey,wu2005coding,unterweger2013compression,
zeng2014characterizing} and stereoscopic
3D~video~\cite{boev2008classification,boev2009stereoscopic,hanhart20133d}, to
the best of the authors' knowledge, there has not been such a review on
artifacts related to end-to-end 360-degree content.
%%
\cite{knorr2017modular} is the only work that provides a preliminary
discussion on the artifacts related to 360-degree content, but it is limited
to capturing artifacts, and does not include an end-to-end analysis that
includes coding, transmission, rendering, and display.

Recently, there has been some effort on measuring the visual quality of
360-degree video~\cite{%
  ebrahimi2017measuring,
  schatz2017towards,
  duan2018perceptual,
  lim2018vr,
  xu2017visual,
  zhang2018subjective,
  zou2018perceptual%
}.
%%
None of them, however, is based on the analysis of perceptual artifacts.
%%
In this paper, we aim at filling this gap by providing an overview of the
perceptual artifacts in current 360-degree video processing pipelines.
%%
Such a contribution may also help in providing the basis for new and more
perceptual correct objective visual quality metrics for 360-degree content,
which take into account and quantify the perceived artifacts.

The remainder of the paper is organized as follows.
%%
Section~\ref{sec:360pipeline} presents a common 360-degree pipeline, used by
most of the state-of-the-art approaches.
%%
Section~\ref{sec:360artifacts} details for each step of the 360-degree
pipeline the common artifacts that have visual manifestation.
%%
Section~\ref{sec:discussion} discusses the current approaches and the open
issues on the visual quality of 360-degree video.
%%
Finally, Section~\ref{sec:conclusion} brings our conclusions and points out
future work on how to use the comprehensive review to improve current
360-degree object quality metrics and as means of compensating for the
artifacts.


